On Training Derivative-Constrained Neural Networks

We refer to the setting where the (partial) derivatives of a neural network's (NN's) predictions with respect to its inputs are used as additional training signal as a derivative-constrained (DC) NN. This situation is common in physics-informed settings in the natural sciences. We propose an integrated RELU (IReLU) activation function to improve training of DC NNs. We also investigate denormalization and label rescaling to help stabilize DC training. We evaluate our methods on physics-informed settings including quantum chemistry and Scientific Machine Learning (SciML) tasks. We demonstrate that existing architectures with IReLU activations combined with denormalization and label rescaling better incorporate training signal provided by derivative constraints.

==> dustbin.tex <==
% We study neural network (NN) training in the setting where derivatives of the NN with respect to its inputs are used to express constraints on its predictions. We call this scenario \emph{derivative-constrained machine learning} (DCML). DCML is common in constructing machine learning (ML) models of natural processes (e.g., in chemistry, physics, biology) where gradients of the model are used to express physical constraints (e.g., conservation of energy). While it is possible to construct NNs with high predictive accuracy using standard techniques in DCML, we may do so at the cost of satisfying gradient constraints. 

% Models of natural processes (e.g., in chemistry, physics, biology) often involve gradients of the model to express constraints (e.g., conservation of energy). We call machine learning (ML) in this setting with gradient constraints \emph{gradient-constrained machine learning} (DCML). In spite of the high predictive accuracy of many DCML models, it may do so at the cost of satisfying its gradient constraints. This highlights a need to reevaluate aspects of DCML training, including data preprocessing, regularization, and architecture. We explore dataset scaling, denormalization, and a new activation function called an integrated RELU activation to improve DCML training. We demonstrate our methods on quantum chemistry and Scientific Machine Learning (SciML) tasks.

% Gradient-constrained machine learning (DCML) merges traditional machine learning (ML) with modeling data possessing inherent derivative relationships, often stemming from natural processes like physics or chemistry. These processes, described by partial differential equations, dictate constraints on DCML models. However, despite the high predictive accuracy of modern DCML models, it struggles to produce equally precise derivatives.





% DL mostly for computer vision and NLP
% Deep learning has demonstrated successes in many fields, most prominently in computer vision~[cite] and natural language processing~[cite]. Many common neural network (NN) design patterns and training procedures, including architectures (e.g., activation functions) and regularization techniques (e.g., batch normalization~[cite]) have been developed in these contexts. As deep learning is applied across a broader set of applications, we may need to revist best practices to handle domain requirements.


% % What is gradient-constrained ML?
% Natural processes (e.g., in physics and chemistry) are described by partial differential equations (PDEs) which impose constraints on the model in the form of its (partial) derivatives. Typically, we encode these derivative constraints as loss terms in a multi-objective loss function. The field of Scientific Machine Learning (SciML) is emerging to address the issues of applying ML to the physical sciences (\eg physics-informed neural networks or PINNs). More broadly, we refer to ML in the setting where there are gradient constraints as \emph{gradient-constrained machine learning} (DCML).

% Models of natural processes (e.g., in physics and chemistry) often involve gradients of the model to express constraints (e.g., conservation of energy). We call ML in this setting \emph{gradient-constrained machine learning} (DCML).


% Gradient-constrained machine learning (DCML) is emerging as a discipline to bring the success of traditional machine learning (ML) to model datas which we could find derivative relationships inside. Such datas are usually generated by natural processes (\eg, physical, chemical, biological). Natural processes are described by partial differential equations (PDEs) which impose constraints on the model in the form of its (partial) derivatives. Typically, we would find those derivative constraints applied in CGML training as loss terms in a multi-objective loss function. One of the best known application of DCML is Scientific machine learning (SciML), which naturally involves computing higher-order derivatives (\eg physics-informed neural networks (PINNs)).  

% However, DCML models generally suffer from high error of its model gradient. Given the high quality predictions that nowadays neural networks (NNs) can produce, DCML models which specialized on gradient fitting are still falling short to give precise derivatives on the same level as its prediction \ref{evidance}. As a result, current design patterns may not bring DCML further. This means that there is an opportunity to revisit parts of the training designs: dataset preprocessing, model architecture, and regularization.


\begin{comment}
    However, models in SciML still use standard activation functions (\eg, RELU~\cite{agarap2018deep}) that are used when training with standard procedures that use first-order derivatives. An activation function such as a RELU has a vanishing second-order derivative. Consequently, we may lose signal when training NNs using this activation function when higher-order derivatives are involved (Section~\ref{sec:problem}). This may impact the quality of training, which may make it more difficult to realize the benefits of ML in the physical sciences. Compared to typical use cases of ML where only first-order derivative information is used, it is also understudied what activation functions, architectures, and training procedures to use in the setting when higher-order derivatives are required.
\end{comment}



% % % Why are we applying ML to science? What are the benefits?
% 

% Natural processes are described by partial differential equations (PDEs). PDEs impose constraints on the model in the form of its (partial) derivatives. Consequently, the construction

% As we apply deep learning to a broader set of applications, we may find that we need to revisit common NN design and training choices.

% What is DCML?
% In this paper, we consider the setting of NN training where derivatives of a NN model with respect to (w.r.t.) its inputs are used to express constraints on its predictions. 

% Why DCML?
% DCML is common in constructing machine learning (ML) models of natural processes (e.g., in chemistry, physics, biology). Natural processes are described by partial differential equations (PDEs) which imposes constraints on the model in the form of its (partial) derivatives. Scientific Machine Learning (SciML) is emerging to address the issues of applying ML to the physical sciences (\eg, physics-informed neural networks or PINNs~[cite]). DCML thus addresses a subset of the issues addressed by SciML. 
% As deep learning is applied to these settings, developing best practices for DCML will become increasingly important.




% and density functional theory (DFT). These simulations are compute-intensive, but they motivates a data-driven approach. The negative gradient of a PES $-\nabla U: \R_{pos}^{3A} \rightarrow \R_{F}^{3A}$ gives the forces acting on an atomistic system and can be used to simulate the dynamics of a system. 

% Suppose we have a dataset $(x^i, E^i, F^i)_i$ where $x^i$ encodes the atomic coordinates, $E^i$ is the energy, and $F^i$ is the force. 


%Higher-order derivative information enters the training of a NN with this loss function since the derivative of the NN w.r.t. the parameters $\theta$ is a second-order derivative. 



% In the physics-aware setting, the inputs $\mathbf{x}^i$ correspond to the description of a physical configuration such as the position of atoms. The outputs $y^i$ correspond to physical observables such as energies. The relationship between configurations and observables is often expressed using partial differential equations (PDEs). PDEs express relationships between variables using (partial) derivatives.

% A function $f_\theta(x) = y$ would then be a \emph{potential energy} function. The negative gradient $\nabla_\mathbf{x} f_\theta$ would then be the force applied to the system.

% The \emph{derivative-constrained machine learning} (DCML) setting additionally considers the inclusion of derivative constraints on the model. For example, we can add the constraint that $\frac{\partial}{\partial \mathbf{x}_i} f_\theta = \mathbf{x}_i^2$ so that the partial derivatives of the model $f_\theta$ w.r.t. the input $\mathbf{x}_i$ are equal $\mathbf{x}_i^2$. This derivative constraint can be encoded as a loss term in a multi-objective loss term
% \begin{equation}
%     L(f_\theta, \cD) = \sum_{i=1}^N \alpha \lVert f_\theta(\mathbf{x})^i - y^i \rVert^2 + \beta \lVert \nabla_\mathbf{x} f_\theta(\mathbf{x}^i) - (\mathbf{x}^i)^2 \rVert^2
% \end{equation}
% where $\alpha$ and $\beta$ control the importance of each term. It is straightforward to encode other higher-order derivatives and more terms.

% Derivatives of the model can also be given as additional supervision signal. For example, consider a dataset $\cD = (\mathbf{x}^i, (y^i, \mathbf{g}^i))_{i}$ which additionally contains gradient information $\mathbf{g}^i$. This information can also be incorporated into a multi-objective loss function
% \begin{equation}
%     L(f_\theta, \cD) = \sum_{i=1}^N \alpha \lVert f_\theta(\mathbf{x})^i - y^i \rVert^2 + \beta \lVert \nabla_\mathbf{x} f_\theta(\mathbf{x}^i) - \mathbf{g}^i \rVert^2 \,.
% \end{equation}



% While it is possible to construct NNs with high predictive accuracy using standard techniques in the example above, care must be taken. 

% since we have two interrelated challenges: (1)  (1) scale-aware and (2)


% 

% Unlike common ML tasks such as image classification, DCML is not scale invariant. This introduces two interrelated challenges: (1) handling units and (2) handling magnitude differences between predictions of the model and gradients of the model.

% In a typical setting, 

% While this solves the problem of handling units, it does not solve the problem of handling magnitude difference between predictions of the model and derivatives of the model. 

% More generally, we might hope to improve the situation by improving the NN architecture $f_\theta$.

% For example, in a typical setting, we can apply ML to unit-less datasets by normalizing the dataset. Such a step is also practically important to ensure numerical stability of training. However, upon inspection of the loss terms above, we can see that it is not possible to directly apply dataset normalization. Let $n(\mathbf{x})$ normalize a datapoint. Then by a basic application of the chain rule, we see that we also need to consider the transformed variable, resulting in a loss function
% \begin{equation}
%     L(f_\theta, \cD) = \sum_{i=1}^N \alpha \lVert f_\theta(n(\mathbf{x})^i) - y^i \rVert^2 + \beta \lVert \nabla_\mathbf{x} f_\theta(n(\mathbf{x}^i)) \nabla n(\mathbf{x}^i) - (\mathbf{x}^i)^2 \rVert^2 \,.
% \end{equation}


% NNs can be used to model the PES of an atomistic system in the domain of quantum chemistry. 
% mean energy loss and mean force loss on datasets of molecule conformations (\ie, different orientations of the same molecule). 
%Schnet is a convolution based NN while the other works are graph neural network (GNN). CGCNN is an advanced version of GNN which interprets crystal structures as graphs. Dimenet++ is a multi-pathed GNN with 4 branches in the end of model's structure. 
% Forcenet is a GNN which features encoder-decoder architecture. 


% However, upon some reflection, this might leave a lot to be desired since we are implicitly setting the units of the inputs and outputs to control the relative importance of each term. For example, $\alpha = 1$ and $\beta = 1000$, to be concrete, would mean that we are predicting position using Angstroms (a measure of distance) and forces in units of kilo-electron volts per Angstrom (a unit of force).


% Thus, physics-aware training forms one aspect of constructing models of natural phenomenon as in SciML.

% Physics-aware training has two features that set it apart from traditional ML. First, 


% It is important to efficiently incorporate derivative constraints during training in physics-aware settings to properly incorporate physics knowledge.


% Second, physics-aware models are \emph{scale-aware}. For example, the physical properties of a molecule (\ie, a structure) whose atoms are twice as far apart are different than those of a molecule whose atoms are unscaled. In contrast, an image classification task is invariant to the scale of the image and natural language tasks do not have a meaningful notion of scale. 


% We demonstrate that this occurs in the setting of potential energy surface (PES) modeling in quantum chemistry (Section~\ref{sec:pam}).


% However, physics-aware modeling is scale-aware. Consequently, normalizing the features in a standard way may introduce non-physical artifacts into the learning process.

% Continuing this line of reasoning, we may then wonder if normalization within a NN architecture such as batch normalization~[cite] can be applied in physics-aware modeling. 



% Normalization is commonly used in datasets for machine learning. Using data normalization has several merits like speed up convergence/training, avoid numeric instability and enhance generalize ability. However, In GCML, where data could possess inherent derivative relationships (\eg physic laws), the units of data are required to be preserved for correct semantics of those relationships. Normalizing the data would thus remove the units in data and erase the derivative signals in dataset. This concept can also apply to normalization layers in the model architecture. For the GCML models that are supposed to enhance derivative signals, normalization layers cancels the possible higher-order signals its current input features can hold. 

% To preserve the valuable higher-order signals in the dataset and during model inference, we propose removing all normalization techniques such as data normalization, batch normalization and layer normalization. Since normalization layers in NNs have the same output dimension as input size, we can take the layers out without structural amendment. As for the lost benefits from normalization, we introduce data re-scaling in Sec.~\ref{sec:methods_data_rescaling} to reduce numeric instability and take the others as trade-offs for precision. 




% \subsection{Label Re-scaling}
% \label{sec:methods_data_rescaling}


% More concretely, suppose we have a dataset normalization procedure $n: X \rightarrow X$ that normalizes data. Then a gradient constraint in a loss term
% \begin{equation}
%     \nabla_\mathbf{x} f_\theta(n(\mathbf{x})) = (\nabla_\mathbf{x} n(\mathbf{x}))^T (\nabla_\mathbf{x} f_\theta(n(\mathbf{x})))
% \end{equation}
% needs to be multiplied by $(\nabla_\mathbf{x} n(\mathbf{x}))^T$ to ensure proper scaling by the chain-rule.

==> sections/other/Experiments_og.tex <==
\section{Experiments}
\label{sec:experiments}
This section presents the performance of our proposed method tested across domains of dataset and architecture. The hardware detail, datasets and scripts we used are available in supplementary material.

\subsection{Quantum Chemistry}
\label{sec:experiments_qc}
% quick review of DC in QC dataset metioned in motivation
From Sec.~\ref{sec:DCmodeling_setup}, we explained DC modeling in quantum chemistry is a task mapping atomic coordinates in a molecule $\R^{3A}$ to its system energy $\R$. Besides the predictive loss (energy loss), the loss function also involves derivative loss (force loss) as its physics constraint which tells: the force field is the negative gradient of the potential energy surface w.r.t. atomic positions. With this derivative constraint, we test the effectiveness of our proposed methods in domain of quantum chemistry. 

% methology
The NNs in the experiments of quantum chemistry (Sec.~\ref{sec:experiments_qc_ir}, Sec.~\ref{sec:experiments_qc_denorm} and Sec.~\ref{sec:experiments_qc_joint}, Sec.~\ref{sec:experiments_qc_sclaing}) are trained 50 epochs with MD17 dataset, batch size 20, Adam optimizer and initial learning rate 0.0001. Given the fast convergence of the training loss in MD17, we consider 50 epochs is sufficient for models to fully learn the energy and forces. 
For each molecule in MD17, we randomly select 50000, 6250 and 6250 conformations from the trajectory as training set, validation set and testing set. Baseline models are trained with the same training configuration and model hyperparameters used by Project OCP. 

% experiment spec
For the sake of paper arrangement, in the experiment tables, we abbreviate the name of the 8 molecules in MD17 presented by take their first three letters. We provide the abbreviation table in Appendix. In each cell in the tables, energy loss (kcal/mol) is presented on the upper row and force loss (kcal/mol/\AA) is presented on the bottom row.

\subsubsection{Result}
\label{sec:experiments_qc_joint}
% additional methology section
From Sec.~\ref{sec:methods_integrated_relu} and Sec.~\ref{sec:methods_de_normalization}, we have specified the formulation of our proposed methods respectively. To demonstrate the overall effectiveness of our proposed methods, we trained variety of SOTA models: SchNet, CGCNN, ForceNet, DimeNet++, GemNet with both integrated ReLU, denormalization and label rescaling applied (for models with normalization layers, we still apply rescaling). In Tab.~\ref{tab:exp_qc_joint}, we show the performance of comparison between the models trained with original settings and trained with the joint effort of our proposed methods. For label rescaling, we use constant $k=1000000$ by heuristic. The results of joint efforts are noted with * in the table. 

% result
The result of Tab.~\ref{tab:exp_qc_joint} shows that with integrated ReLU, denormalization and label rescaling, performances of CGCNN, DimeNet++ and FroceNet complete dominate their original setting. Also, in terms of overall energy loss, the improved models have consistent (38 out of 40) better performance in all the architectures tested. For force losses, our proposed methods show significant improvement in CGCNN, DimeNet++ and ForceNet. In the other hand, when our approaches do not perform perfectly ideal, the models (SchNet and GemNet) at least maintain close force losses compare to original settings.

\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
        \hline
        Model & Asp. & Ben. & Eth. & Mal. & Nap. & Sal. & Tol. & Ura.\\
        \hline 
        SchNet   & 53.008 & 125.432 & \textbf{5.974} &  37.542 & 197.062 & 65.466 & 129.806 & 54.882 \\
                 & \textbf{1.216}  & 0.390   & \textbf{0.685}  &  \textbf{1.006}   & \textbf{0.721}   & \textbf{1.026}   & \textbf{0.672}   & \textbf{0.867}  \\
        \hline 
        SchNet*  & \textbf{28.316} & \textbf{0.566} & 13.393 &  \textbf{11.278} & \textbf{5.536} & \textbf{27.573} & \textbf{0.343} & \textbf{20.361} \\
                 & 1.672  & \textbf{0.369}   & 1.531  &  1.670   & 1.011   & 1.120   & 1.046   & 1.234  \\
        \hhline{|=|=|=|=|=|=|=|=|=|} 
        CGCNN    & 239.078 & 98.867 & 38.362 &  104.456 & 130.984 & 197.096 & 124.290 & 133.517 \\
                 & 14.206  & 6.119   & 8.251  &  14.273   & 8.466   & 8.500   & 9.730   & 9.081  \\
        \hline 
        CGCNN*   & \textbf{137.125} & \textbf{16.634} & \textbf{4.639} &  \textbf{30.568} & \textbf{66.681} & \textbf{78.299} & \textbf{36.736} & \textbf{81.020} \\
                 & \textbf{7.132}  & \textbf{0.615}   & \textbf{2.969}  &  \textbf{4.997}   & \textbf{2.389}   & \textbf{4.776}   & \textbf{2.912}   & \textbf{4.934}  \\
        \hhline{|=|=|=|=|=|=|=|=|=|} 
        DimeNet++   & 47.437 & 133.701 & 236.942 &  856.015 & 1096.34 & 580.416 & 301.061 & 669.067 \\
                    & 13.826  & 12.452   & 6.411 &  8.870   & 7.820   & 10.412   & 8.646   & 6.156  \\
        \hline 
        DimeNet++*  & \textbf{2.598} & \textbf{1.686} & \textbf{0.589} & \textbf{20.304} & \textbf{5.184} & \textbf{3.651} & \textbf{0.773} & \textbf{5.965}\\
                    & \textbf{2.521}  & \textbf{0.255}   & \textbf{0.296}  &  \textbf{0.787}   & \textbf{0.706}   & \textbf{1.792}   & \textbf{0.464}   & \textbf{0.715}  \\
        \hhline{|=|=|=|=|=|=|=|=|=|} 
        FroceNet   & 755.490 & 239.531 & 1048.44 & 874.220 & 1677.710 & 165.174 & 369.338 & 1964.510 \\
                   & 21.955  & 117.793   & 17.612  & 31.525 & 18.160 & 22.364 & 18.334 & 46.477  \\
        \hline 
        ForceNet*  & \textbf{13.802} & \textbf{19.092} & \textbf{3.185} & \textbf{4.525} & \textbf{5.980} & \textbf{41.437} & \textbf{5.634} & \textbf{14.548} \\
                   & \textbf{0.895} & \textbf{0.332} & \textbf{1.150} & \textbf{1.368} & \textbf{0.358} & \textbf{0.341} & \textbf{0.507} & \textbf{0.262}  \\
        \hhline{|=|=|=|=|=|=|=|=|=|} 
        GemNet   & 2201.94 & 352.19 & 470.324 & \textbf{5.236} & 564.068 & 1238.93 & 193.501 & 228.105 \\
                 & \textbf{0.349}  & \textbf{0.225}   & 0.289  &  \textbf{0.274}   & \textbf{0.175}   & \textbf{0.307}   & \textbf{0.122}   & \textbf{0.208}  \\
        \hline 
        GemNet*  & \textbf{13.162} & \textbf{6.311} & \textbf{7.101} &  15.366 & \textbf{5.874} & \textbf{5.676} & \textbf{8.136} & \textbf{21.981} \\
                 & 0.938 & 1.275 & \textbf{0.270} & 0.700 & 0.479 & 0.735 & 0.471 & 7.076 \\
        \hline
    \end{tabular}
    \caption{Comparison of model performance trained with original setting and our proposed methods. Mean energy loss (kcal/mol) on the upper row and mean force loss (kcal/mol/\AA) on the bottom row of the eight molecules in MD17 trained on state-of-the-art models. The models are trained on single molecule training set in MD17 and tested on their corresponding testing set.}
    \label{tab:exp_qc_joint}
\end{table}

\subsubsection{Scaling On Data}
\label{sec:experiments_qc_sclaing}
% additional methology section
In quantum chemistry domain, a significant reason shifting from traditional simulation approaches to NNs is their scalability difference. Applied with both our proposed methods, we expect the improved models can maintain the scalability merit of NNs', showing progressively better performance as the amount of data increases. In this section, we experiment SchNet with integrated ReLU, label rescaling ($k=1000000$) on different amount of input data:{50000, 100000, 150000, 200000}, reported in Fig.~\ref{fig:exp_qc_scaling} \footnote{Limited by the amount of conformations provided in MD17, Aspirin trajectory does not have enough sample to test on scale: 150000, 200000. Uracil trajectory does not have enough sample to test on scale: 200000.}. 

% result
Fig.~\ref{fig:exp_qc_scaling} proves as amount of samples in training set increases, losses in both energy and forces consistently decrease. Our proposed methods, as a result, have ability to train on more data when traditional methods would suffer a lot from it. Given it is possible to train on more data, simulations in the field of quantum chemistry can thus have better accuracy in the same task.  

\begin{figure}[t]
    \centering
    \begin{subfigure}{.4\textwidth}
        \centering
        \includegraphics[scale=0.4]{figures/scalingE.png}
        \caption{scalability on energy}
        \label{fig:betas:train}
    \end{subfigure}
    \hskip 2em
    \begin{subfigure}{.4\textwidth}
        \centering
        \includegraphics[scale=0.4]{figures/scalingF.png}
        \caption{scalability on force}
        \label{fig:betas:test}
    \end{subfigure}
    \caption{SchNet trained on MD17 with label rescaling and IReLU. Limited by the amount of conformations provided in MD17, Aspirin trajectory does not have enough sample to test on scale: 150K, 200K. Uracil trajectory does not have enough sample to test on scale: 200K.}
    \label{fig:exp_qc_scaling}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PINN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Physics-informed Neural Networks}
\label{sec:experiments_pinns}

% To test generalizaton ability, we test on PINNs and breif intro to PINNs
To validate the generalize ability of our proposed methods in other domains, aside from quantum chemistry, we also experiment on physics-informed neural networks (PINNs)~\citep{raissi2019physics}. PINNs are a general family of models that use NN to simulate the latent function $\psi(x, t)$ which governs their observation (\eg temperature, velocity) w.r.t coordinate and time. To learn the latent function, PINNs enforce laws of physical dynamics given by PDEs in the loss function. PINNs thus naturally inherent derivative constraints in its setting. Different from the tasks in quantum chemistry (Sec.~\ref{sec:DCmodeling}), instead of producing gradients losses as part of the metric, PINNs only evaluate performances on predictive accuracy. Also, in some PINNs (ref), their PDE could manipulate derivatives that has order of two or more.    

% DC constraints in PINNs
The loss function of PINNs consists multiple loss terms. We can categorize them into three major groups: (1) PDE loss (f loss), which involves higher order derivatives of the model, initial condition loss (IC loss) which governs values when time=0 and boundary condition loss (BC loss) which governs the values on the geometry boundary of data. Combined, the loss function gives: 

\begin{equation}
\mathcal{L}(\mathcal{T})= \mathcal{L}_f\left( \mathcal{T}_f\right)+\mathcal{L}_{ICBC}\left( \mathcal{T}_i, \mathcal{T}_b \right)
\end{equation}

\begin{equation}
\mathcal{L}_f\left(\mathcal{T}_f\right)=\frac{1}{\left|\mathcal{T}_f\right|} \sum_{\mathbf{x} \in \mathcal{T}_f}\left\|f\left(\mathbf{x} ; \frac{\partial \psi}{\partial x_1}, \ldots, \frac{\partial \psi}{\partial x_d} ; \frac{\partial^2 \psi}{\partial x_1 \partial x_1}, \ldots, \frac{\partial^2 \psi}{\partial x_1 \partial x_d} ; \ldots ; \boldsymbol{\lambda}\right)\right\|_2^2
\end{equation}

\begin{equation}
\mathcal{L}_{ICBC}\left(\mathcal{T}_i, \mathcal{T}_b\right)= \frac{1}{\left|\mathcal{T}_i\right|} \sum_{\boldsymbol{x} \in \mathcal{T}_i}\|\mathcal{I}(\psi, \mathbf{x})\|_2^2 + \frac{1}{\left|\mathcal{T}_b\right|} \sum_{\boldsymbol{x} \in \mathcal{T}_b}\|\mathcal{B}(\psi, \mathbf{x})\|_2^2 
\end{equation}

where $\mathcal{T}$ is the training set which is separated into $\mathcal{T}_f$, $\mathcal{T}_{i}$ and $\mathcal{T}_{b}$ for the three groups of loss terms. $\psi$ is the latent function simulated by the NN that governs the behavior of physic. $\psi$ takes geometry (1D, 2D or 3D coordinate) and time as inputs. $\lambda$ is the coefficient for each partial derivative in f loss. $\mathcal{I}$ is the initial condition function that decides the values when time=0 and $\mathcal{B}$ is the boundary condition function that decides the values on geometry boundary.

Notice that there could be multiple IC, BC loss terms and IC, BC loss could also involve higher-order derivatives in certain PINNs. Here we experiment on four different PINNs that are highly reproducible from PDEBench\citep{PDEBench2022,darus}, a well-known public work that provides implementation and benchmark of SciML models including PINNs: advection equation, compressible fluid dynamic equation, shallow water equation and diffusion-reaction equation.  

For experiments of PINNs, we adapt baseline architectures, datasets and training configurations from PDEBench. In the baseline architecture, all the PINNs use the same MLP with 6 hidden layers of 40 neurons in each to simulate their latent function $\psi$. The MLP uses Tanh activation function for every hidden layer. We use the same library DeepXDE~\citep{lu2021deepxde} to construct and train the backbone MLP.

\subsubsection{Advection Equation}
\label{sec:experiments_pinns_adv}
% methodology
For advection equation, we experiment training with/without batch normalization layers and with/without IReLU. Both models are trained 15000 epochs on the training set of 1D Advection dataset ($\beta=0.1$) from PDEBench with Adam optimizer, initial learning rate=$0.001$. The full loss function associated with the advection equation is presented in the supplementary material.

% results
Advection equation is a basic PINN to learn. It has a simple PDE in $f$ loss, exactly one initial condition and boundary condition. In Tab.~\ref{tab:exp_pinns_adv}, we present the predictive loss evaluated in testing set and training loss of each term in the multi-objective loss function evaluated in the last epoch of training. Loss terms with $\dagger$ are the terms which involve higher order derivatives. Combined with IReLU and denormalization, model achieves the best performance in predictive metirc and also significant improve with two of the training loss terms. More, by comapring $f$ loss, we show our proposed methods can effectively preserve higher-order derivative signal in training phase.  

\begin{table}[t] 
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        Model & $pred$ & $f^\dagger$ & $IC$ & $BC$ \\
        \hline 
        Tanh+bn     & 1.701 & 8e-16 & 5e-5  & 3e-5 \\
        \hline 
        IReLU+bn    & 2.424 & 9e-12 & 8e-6  & 2e-6 \\
        \hline
        Tanh+denorm & 1.594 & 1e-5  & \textbf{3e-6}  & 6e-6 \\
        \hline
        IReLu+denorm& \textbf{0.991} & \textbf{$<$e-45} & 0.088 & \textbf{$<$e-45} \\
        \hline
    \end{tabular}
    \caption{MSE of loss terms of advection equation. $pred$ is the predictive loss. $f$ is the loss of the PDE which governs advection equation. $IC$ is the loss of initial conditions and $BC$ is the loss of boundary conditions.}
    \label{tab:exp_pinns_adv}
\end{table}


\subsubsection{Compressible Fluid Dynamic Equation}
\label{sec:experiments_pinns_CFD}
% methodology
For CFD equation, both models are trained 15000 epochs on training set of 1D CFD dataset ($\eta=10^{-8}, \zeta=10^{-8}$) from PDEBench with Adam optimizer, initial learning rate=$0.001$. The full loss function associated with the CFD equation is presented in the supplementary material.

% results
CFD equation is advanced from advection function. It has totally 6 initial and boundary conditions. With the same weight on each loss term, the equivalent ratio of weight on gradient loss and prediction loss becomes 1:6. It challenges the NN's ability to fit gradient under such disadvantage. In Tab.~\ref{tab:exp_pinns_cfd}, we present the predictive loss evaluated in testing set and training loss of each term in the multi-objective loss function evaluated in the last epoch of training. Loss terms with $\dagger$ are the terms which involve higher order derivatives. With IReLU and denormalization, the model not only performs the best in predictive metirc, it also surpasses the other models in all the training loss terms. For the term involving derivatives ($f$ loss), our model beats original settings by 4 orders.   

\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
        \hline
        Model & $pred$ & $f^\dagger$ & $IC_p$ & $IC_d$ & $IC_v$ & $BC_p$ & $BC_d$ & $BC_v$ \\
        \hline 
        Tanh+bn       & 1.119 & 271.944 & 2910.327 & 11.373 & 0.258 & 0.156 & 0.156 & 0.156 \\
        \hline 
        IReLU+bn      & 1.664 & 2e+7    & 4656.733 & 32.972 & 0.878 & 1.963 & 1.963 & 1.963 \\
        \hline
        Tanh+denorm   & 0.870 & 7.962   & 4694.601 & 16.016 & 0.273 & 0.111  & 0.111  & 0.111 \\
        \hline
        IReLu+denorm  & \textbf{0.407} & \textbf{0.110}   & \textbf{88.788}   & \textbf{0.211}  & \textbf{0.176} & \textbf{1e-6}  & \textbf{1e-6}  & \textbf{1e-6} \\
        \hline
    \end{tabular}
    \caption{MSE of loss terms of CFD equation. $pred$ is the predictive loss. $f$ is the loss of the PDE which governs CFD equation. $IC_p$, $IC_d$, $IC_v$ are the loss of initial conditions of pressure, density, velocity respectively. $BC_p$, $BC_d$, $BC_v$ are the loss of boundary conditions of pressure, density, velocity respectively.}
    \label{tab:exp_pinns_cfd}
\end{table}


\subsubsection{Diffusion Reaction equation}
\label{sec:experiments_pinns_diffreact}

% methodology
For the diffusion reaction equation, both models are trained for $100$ epochs on the training set of 2D diff-react dataset ($1000$ samples) from PDEBench with the Adam optimizer and an initial learning rate=$0.001$. The full loss function associated with the diffusion reaction equation is presented in the supplementary material.

% results
In the diffusion-reaction experiment, second order derivative is involved in its PDE, which implies third order derivative information would be processed during NN trianing. Also, there are Neumann boundary conditions which utilize gradient information to describle problem's boundary state in each given time step. In Tab.~\ref{tab:exp_pinns_diffreact}, we present the predictive loss evaluated in testing set and training loss of each term in the multi-objective loss function evaluated in the last epoch of training. Loss terms with $\dagger$ are the terms which involve higher order derivatives. With IReLU and denormalization, the models has the best predictive loss and also the best and second best in training loss terms which involves higher order. This experiment demonstrates that our proposed methods has ability to fit gradients of NN that have order more than two. 

\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|}
        \hline
        Model & $pred$ & $f^\dagger$ & $IC_u$ & $IC_v$ & $BC^\dagger$ & $BC_u$ & $BC_v$\\
        \hline 
        Tanh+bn      & 4.946 & 0.469 & 1.184 & 1.062 & \textbf{2e-15} & 0.083 & 0.008\\
        \hline 
        IReLU+bn     & 8.037 & 7e+4  & 0.989 & 1.005 & 2e-10 & 4.445 & 4.344\\
        \hline
        Tanh+denorm  & 1.354 & 2e-4  & \textbf{0.978} & \textbf{0.999} & 1e-4  & \textbf{1e-4}  & \textbf{3e-5}\\
        \hline
        IReLu+denorm & \textbf{1.130} & \textbf{1e-4}  & 0.980 & 1.001 & 3e-14 & 0.004 & 3e-4\\
        \hline
    \end{tabular}
    \caption{MSE of loss terms of diffusion-reaction equation. $pred$ is the predictive loss. $f$ is the loss of the PDE which governs diffusion-reaction equation. $IC_u$, $IC_v$ are the loss of initial conditions of activator and inhibitor respectively. $BC$ is the loss of derivative of boundary conditions. $BC_u$, $BC_v$ are the loss of boundary conditions of activator and inhibitor respectively.}
    \label{tab:exp_pinns_diffreact}
\end{table}

\begin{comment}
\subsubsection{Shallow Water Equation}
\label{sec:experiments_pinns_swe}

% methodology
For SWE equation, both models are trained 15000 epochs on the training set of 2D SWE dataset (1000 samples) from PDEBench. with Adam optimizer, initial learning rate=$0.001$. The full loss function associated with the SWE equation is presented in the supplementary material.
\end{comment}
    


